SRT22 does not imply RT22 in omega-models

We complete a 40-year old program on the computability-theoretic analysis of Ramsey's theorem, starting with Jockusch in 1972, and improving a result of Chong, Slaman and Yang in 2014. Given a set $X$, let $[X]^n$ be the collection of all $n$-element subsets of $X$. Ramsey's theorem for $n$-tuples asserts the existence, for every finite coloring of $[\omega]^n$, of an infinite set $X \subseteq \omega$ such that $[X]^n$ is monochromatic. The meta-mathematical study of Ramsey has a rich history, with several long-standing open problems and seminal theorems, including Seetapun's theorem in 1995 and Liu's theorem in 2012 about Ramsey's theorem for pairs. The remaining question about the study of Ramsey's theorem from a computational viewpoint was the relation between Ramsey's theorem for pairs ($\mathsf{RT}^2_2$) and its restriction to stable colorings ($\mathsf{SRT}^2_2$), that is, colorings admitting a limit behavior. Chong, Slaman and Yang first proved that $\mathsf{SRT}^2_2$ does not formally imply $\mathsf{RT}^2_2$ in a proof-theoretic sense, using non-standard models of reverse mathematics. In this article, we answer the open question whether this non-implication also holds within the framework of computability theory. More precisely, we construct a $\omega$-model of $\mathsf{SRT}^2_2$ which is not a model of $\mathsf{RT}^2_2$. For this, we design a new notion of effective forcing refining Mathias forcing using the notion of largeness classes.

==> parts/part3-extensions.tex <==

We prove that given a Turing functional $\Gamma$, for every set $A$, there is an infinite subset $G \subseteq A$ or $G \subseteq \overline{A}$ such that $\Gamma^{G'}$ is not a completion of $n \mapsto \Phi^{\emptyset}_n(n)$.

Let $A^0 = A$ and $A^1 = \overline{A}$.
Fix a $\Delta_0$ formula $\Phi_e(G, x, y, p)$ with two integer variables $x$ and $y$, and a valuation variable $p$.
Let $W$ be the $\emptyset'$-c.e. set of all valuations $p$ such that for every $Z^0 \cup Z^1 = \omega$, the collection
$$
\Acal_p = \Lcal_\omega \bigcap \{ \Ucal_{\zeta(e, \rho, x, p)} : i < 2, \rho \subseteq Z^i, x \in \omega \}
$$
is not an acceptability class, where
$$
\Ucal_{\zeta(e, \rho, x, p)} = \{ X : (\rho, X) \not \Vdash (\forall y)\Phi_e(G, x, y, p)\}
$$
By \Cref{lem:combi-liu-valuation}, either there is a $\emptyset'$-correct valuation belonging to $W$, or there are 11 pairwise incompatible valuations outside $W$.

\bigskip
Case 1: $p \in W$ for some $\emptyset'$-correct valuation. Then letting $Z^0 = A^0$ and $Z^1 = A^1$, there is a low cover $X_0 \cup \dots \cup X_{k-1} = \omega$ such that for every $j < k$, $X_j \not \in \Acal_p$.
Let $j < k$ be such that $X_j \in \Lcal_\omega$ (in other words $X_j$ infinite). Then there is some $i < 2$, some $\rho \subseteq A^i$ and some $x \in \omega$ such that $X_j \not \in \Ucal_{\zeta(e, \rho, x, p)}$. In $X_j \cap A^i$ is finite, then the set $G = X_j - A_i$ is an infinite subset of $A^{1-i}$ of low degree, and are we are done. Otherwise, $G = \rho \cup (X_j \cap A_i)$ is an infinite subset of $A^i$ such that $(\exists x)(\forall y)\Phi_e(G, x, y, p)$ holds for some correct valuation $p$, and we are done.

\bigskip
Case 2: there are 11 pairwise incompatible valuations $p_0, \dots, p_{10}$ outside $W$. For every $j < 11$, there is some $Z^0_j \cup Z^1_j = \omega$
such that the class 
$$
\Acal_{p_j} = \Lcal_\omega \bigcap \{ \Ucal_{\zeta(e, \rho, x, p)} : i < 2, \rho \subseteq Z^i_j, x \in \omega \}
$$
is an acceptability class.
For every $j < 11$, either $\Lcal_{Z^0_j} \cap \Acal_{p_j}$ is an acceptability class, or $\Lcal_{Z^1_j} \cap \Acal_{p_j}$ is an acceptability class.
By the pigeonhole principle, there is some $i < 2$ and 5 indices $j_0 < \dots < j_4 < 11$ such that $\Lcal_{Z^i_j} \cap \Acal_{p_j}$ is an acceptability class.

For simplicity, by renaming the colors, let's assume that $i = 0$ and $j_0, \dots, j_4 = 0, \dots, 4$. So for every $j < 5$, $\Lcal_{Z^0_j} \cap  \Acal_{p_j}$ is an acceptability class. Let $\Bcal_{p_j} = \Lcal_{Z^0_j} \cap  \Acal_{p_j}$.

If there is some $j_0 \neq j_1 < 5$ such that $\Lcal_{Z^{j_0}_0} \cap  \Bcal_{p_j}$ is an acceptability class, then by 
 
By the pigeonhole principle, there is some $i < 2$ and 3 indices $r_0 < r_1 < r_2 < 5$ such that $Z^0_0 \in 
